On the connection between the ABS perturbation methodology and differential privacy

This paper explores analytical connections between the perturbation methodology of the Australian Bureau of Statistics (ABS) and the differential privacy (DP) framework. We consider a single static counting query function and find the analytical form of the perturbation distribution with symmetric support for the ABS perturbation methodology. We then analytically measure the DP parameters, namely the $(\varepsilon, \delta)$ pair, for the ABS perturbation methodology under this setting. The results and insights obtained about the behaviour of $(\varepsilon, \delta)$ with respect to the perturbation support and variance are used to judiciously select the variance of the perturbation distribution to give a good $\delta$ in the DP framework for a given desired $\varepsilon$ and perturbation support. Finally, we propose a simple sampling scheme to implement the perturbation probability matrix in the ABS Cellkey method. The post sampling $(\varepsilon, \delta)$ pair is numerically analysed as a function of the Cellkey size. It is shown that the best results are obtained for a larger Cellkey size, because the $(\varepsilon, \delta)$ pair post-sampling measures remain almost identical when we compare sampling and theoretical results.

==> Arxiv 3/macros_arxiv.tex <==
\newcommand{\FigOneTBNoise}[3]
{%\noindent
	\FloatBarrier
\begin{figure*}[!t]
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		{\includegraphics[width=1\columnwidth]{fig1a_arxiv.pdf}}
		\caption{#1} \label{fig:deltasA}   
	\end{subfigure}\hspace{4mm}
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=1\columnwidth]{fig1b_arxiv.pdf}
		%\label{fig:delta1}
		\caption{#2}\label{fig:deltasB}
	\end{subfigure}
	\caption{#3}
	\label{fig:deltas}
\end{figure*}
	\FloatBarrier
}

\newcommand{\FigTwoTBNoiseSupport}[3]
{\noindent
	\FloatBarrier
\begin{figure*}[!t]\begin{subfigure}[t]{0.45\textwidth}
    \centering
             \raisebox{0.40 em}{\includegraphics[width=1\columnwidth]{fig2a_arxiv.pdf}}
            \caption{#1}\label{fig:2A} \end{subfigure}\hspace{4mm}
            \begin{subfigure}[t]{0.47\textwidth}
    \centering
             \includegraphics[width=1\columnwidth]{fig2b_arxiv.pdf}
            \caption{#2}\label{fig:2B} \end{subfigure}
   \caption{#3}
\label{fig:deltaprop3}
\end{figure*}
	\FloatBarrier
}

\newcommand{\FigThreeExampleOne}[1]
{\noindent
	\FloatBarrier
\begin{figure*}[!tbh]
    \centering
             \includegraphics[width=0.6\columnwidth]{fig3_arxiv.pdf}
            \caption{#1}\label{fig:exampl1}
\end{figure*}
	\FloatBarrier
}



==> Arxiv 3/preamble_arxiv.tex <==


%% read in additional TeX-packages or personal macros here:
%% e.g. \usepackage{tikz}
%\usepackage{natbib}
\usepackage[ruled]{algorithm2e}
%\usepackage{bm}
\usepackage{graphicx}
\usepackage{placeins} %FloatBarrier
\graphicspath{{./plots/}} 
%\graphicspath{{plots/}}
\input{macros_arxiv.tex}
%%\input{myMacros.tex}
%% define non-standard environments BEYOND the ones already supplied
%% here, for example
%\theoremstyle{plain}\newtheorem{lemma}[thm]{Lemma}
%% Do NOT replace the proclamation environments lready provided by
%% your own.
\def\eg{{\em e.g.}}
\def\cf{{\em cf.}}
\newcommand{\Ima}{\mathrm{Im}}
\usepackage{subcaption}
\usepackage{amsfonts}
\usepackage{amssymb, amsthm, amsmath}
\usepackage{cite}
\usepackage{tcolorbox}
\usepackage{url}
\def\eps{{\varepsilon}}
\renewcommand{\baselinestretch}{1.1}
\newtheorem{example}{Example}%[section]
\usepackage[margin=1in]{geometry}
\newenvironment{enumerate*}%
{\begin{enumerate}%
		\setlength{\itemsep}{0pt}%
		\setlength{\parskip}{0pt}
		\vspace*{-\topsep}
	}%
	{\end{enumerate}
	\vspace*{-1.5ex}}

\newenvironment{itemize*}%
{\vspace*{0.1ex}
	\begin{itemize}%
		\setlength{\itemsep}{0pt}%
		\setlength{\parskip}{0pt}
		\vspace*{-\topsep}
	}%
	{\end{itemize}
	\vspace*{-1.5ex}
}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary} 
\newtheorem{assumptions}{Assumption} 
\theoremstyle{definition}
\newtheorem{question}{Research Question} 
\newtheorem{defn}{Definition} 
\newtheorem{scheme}{Scheme} 
\newtheorem{remark}{Remark} 

\newcommand{\N}{\mathbb{N}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\CellKey}{\mathtt{KEYSIZE}}
\newcommand{\Rkey}{\mathtt{Rkey}}
\newcommand{\bigN}{\mathtt{bigN}}
\newcommand{\CellVal}{\mathtt{CellKey}}
\newcommand{\PS}{\textcolor{blue}}
\newcommand{\JC}{\textcolor{green}}
